Resource Management in Quantum Virtual Private Networks

In this study, we develop a resource management framework for a quantum virtual private network (qVPN), which involves the sharing of an underlying public quantum network by multiple organizations for quantum entanglement distribution. Our approach involves resolving the issue of link entanglement resource allocation in a qVPN by utilizing a centralized optimization framework. We provide insights into the potential of genetic and learning-based algorithms for optimizing qVPNs, and emphasize the significance of path selection and distillation in enabling efficient and reliable quantum communication in multi-organizational settings. Our findings demonstrate that compared to traditional greedy based heuristics, genetic and learning-based algorithms can identify better paths. Furthermore, these algorithms can effectively identify good distillation strategies to mitigate potential noises in gates and quantum channels, while ensuring the necessary quality of service for end users.

==> extra/background.tex <==
\section{Background and related work}


\subsection{Quantum Background}
% \vspace{-0.02in}
We now briefly mention some of the quantum operations that are relevant to this work.

\myparab{Quantum States:}
A quantum bit (qubit) is fundamentally different than a classical bit. A classical bit can either be in state $0$ or $1$ while a qubit can be in a superposition state of state $0$ and $1.$ Typically a qubit is represented as $|\alpha \rangle= \alpha_1|{0}\rangle +\alpha_2|{1}\rangle$. Similar to one qubit system, a two qubit quantum system can be in a superposition of $|00 \rangle,
|01 \rangle, |10\rangle$, $|11 \rangle$ states and represented as $|\tilde{\alpha} \rangle= \tilde{\alpha}_{1}|{00}\rangle +\tilde{\alpha}_{2}|{01}\rangle+\tilde{\alpha}_{3}|{10}\rangle +\tilde{\alpha}_{4}|{11}\rangle$. While there exists many possible physical realization of a qubit, photonic qubits are most likely to be used for quantum communication and information transfer. In practice, these qubits can be sent through optical fiber based quantum channels using  polarization, time-bin, or absence and presence of a photon based encodings \cite{mattle1996dense}.

%When we measure it, we will get either 0, with probability $|\alpha_1|^2$, or 1, with probability $|\alpha_2| ^2$, where $|\alpha_1|^2+|\alpha_2 |^2=1$. 
%and when we measure it, we will get one of these values: $00,01,10$, or $11$ with probability $|\alpha_{1}|^2,|\alpha_{2}|^2,|\alpha_{3}|^2$ and $|\alpha_{4}|^2$ respectively. 

\myparab{Quantum Entanglement:}
An entangled state is a special type of multi-qubit quantum state which can not be written as the product of its individual component states. The measurement outcomes of an entangled state are correlated. A two-qubit maximally entangled state shared between two parties $A$ and $B$ can be in one of the following four forms, also known as the {\it Bell pairs}: $|\psi_{AB}^{\pm}\rangle=\frac{|{0_A0_B}\rangle\pm|{1_A1_B}\rangle}{\sqrt{2}}$ and $|\phi_{AB}^{\pm}\rangle=\frac{|{0_A1_B}\rangle\pm|{1_A0_B}\rangle}{\sqrt{2}}$. We refer to Bell pair $\ket{\psi_{AB}^+}$ as an Einstein-Podolsky-Rosen {\it (EPR)} pair. 

%$|\psi_{10}\rangle=\frac{|{00}\rangle-|{10}\rangle}{\sqrt[]{2}}$, or $|\psi_{11}\rangle=\frac{|{00}\rangle-|{11}\rangle}{\sqrt[]{2}}$.

%meaning that when we measure the first qubit in a two qubits system, the result of measuring the second qubit is guaranteed to yield the same value or the opposite value. 
\myparab{Entanglement Swapping:}
Suppose two parties $A$ and $B$ share an EPR pair $\ket{\psi_{AB}^+}$. Also, assume that $B$ shares another pair $\ket{\psi_{BC}^+}$ with $C$. Then $B$ can create an EPR pair $\ket{\psi_{AC}^+}$ between $A$ and $C$ by performing a bell state measurement followed by classical communication exchange and a correction. This operation is known as \textit{entanglement swapping}. The process can be repeated in a nested manner to create EPR pairs between distant parties. 

\myparab{Purification:} Due to noisy quantum channels, interaction with the environment, and imperfect quantum operations, the quality of an EPR pair typically decreases from its initial state. However, quantum applications may have a minimum threshold on the fidelity ($F^{th}$) of EPR pairs for subsequent usage. Thus, low-quality EPR pairs delivered to the application may not be suitable for consumption. A quantum operation known as {\it Entanglement Purification} can solve this issue. Entanglement purification typically consumes two low-fidelity base EPR pairs and creates one EPR pair with higher fidelity. Each purification step is probabilistic and both base pairs are lost in case of failure. This operation can be repeated in a nested manner by again purifying  two newly purified EPR pairs until a target fidelity is reached. These protocols are also known as {\it recurrence-based purification protocols}. We refer to a purified EPR pair with fidelity greater than the target fidelity as a high-quality EPR pair.

Let $F$ denote the fidelity of base EPR pairs that participate in purification. The average number $g(F, F^{th})$ of base EPR pairs needed to create one high-quality EPR pair under a recurrence-based purification protocol is given by \cite{Dur1999},
\begin{align}\label{eq:purification_avg}
    g(F, F^{th}) = \prod\limits_{k=1}^{k_{max}}\frac{2}{p_k},
\end{align}
\noindent where $k_{max}$ denotes the number of successful purification steps needed to achieve an output fidelity of $F^{th}$ starting from an input fidelity $F$ and $p_k$ denotes the success probability of $k^{th}$ purification step.

% We first provide two optimization problems where the objective is to maximize a weighted aggregate entanglement generation rate (EGR). They differ according to whether purification is performed by the end nodes or by each link. We also present a third formulation where the objective is to maximize average end-to-end fidelity subject to traffic demands.  Here we only consider the case of end-to-end purification.



==> extra/eval.tex <==
\section{Evaluation}
\label{sec:evaluation}
In this section, we conduct experiments to evaluate different schemes for path selection and answer the following questions: (1) How do different parameters affect the convergence of GA in order to maximize the throughput? (2) Can we guarantee a minimum rate constraint using the genetic algorithm? (3) Can GA find good distillation strategies for each path and for each fidelity threshold in order to mitigate noisy gates? (4) What are the most important factors in the convergence of the GA?


% \begin{table}
%     \centering
%     \setlength{\tabcolsep}{4.6pt}
%     \small
%     \begin{tabularx}{\columnwidth}{L L L L L}
%         \toprule
%         Param & $\cK$  & $w_k (\FORALL{k\in \cK})$& $\lambda^k_u (\FORALL{k\in \cK, u\in U_k})$  & $F^{k}_u (\FORALL{k\in \cK, u\in U_k})$ \\ 
%         \midrule
%         Value & $3$ &Unif$[0.1,1.0]$&Unif$[0.1,1.0]$&Unif$[0.75,0.94]$\\
%         \bottomrule
%     \end{tabularx}
%     \vspace{-0.05in}
%     \caption{\label{tab:parameters_value} Parameters used in our experiments.}
% \end{table}

\myparab{Network topology and workloads:} In our evaluation, we use the Dutch SURFnet network, taken from the Internet topology zoo \cite{zoo}. Physical distance acquired from zoo topology data set \cite{zoo} transmissivity for link of length  = 0.2 dB/km fiber attenuation coefficient link entanglement generation rate:  controls the quality of generated EPR pairs Engineering: Repeaters have been placed between nodes on long links. Parallel links have been added to actual physical 
 links for multiplexing.



Table \ref{tab:parameters_value} shows the value of different parameters used in our experiments.  
We select the flows in the network randomly and set the fidelity threshold of each flow uniformly randomly selected in the range $[0.75,0.94]$. 

% \eat{We set the rate of entanglement generation on each edge in all networks to a value randomly chosen between 200 and 1400.  The fidelity of each edge in the network is randomly chosen from the range [0.96,0.99].
% We set the number of time intervals to 10 ($|T|=10$) and the duration of each time interval ($\Delta$) is 20 seconds.}

\myparab{Purification and Swapping:} We assume all noisy mixed entangled states in the network are Werner states \cite{werner1989quantum}. We compute the basic fidelity of a path as follows:

If we have a path of length $N$ Werner states in a simple linear chain QCN of $N+1$ quantum nodes, the fidelity of the obtained end-to-end entangled link after performing $N$ nested swap operations is given as:

% \begin{equation}\label{eq_nested_swaps_unequal}
% \small
% \begin{split}
%     F = \frac{1}{4} + \frac{3}{4}&{\biggl(\frac{P_2(4\eta^2-1)}{3}\biggl)}^{N-1}\times\biggl(\frac{4F_1-1}{3}\biggl)\\
%     &\times\biggl(\frac{4F_2-1}{3}\biggl)...\biggl(\frac{4F_N}{3}\biggl),
% \end{split}



In our experiments, we use the recurrence-based purification scheme as explained in Section \ref{sec:Preliminaries}. In particular, we use the DEJMPS protocol \cite{Deutsch96} for purification. The values of $p_k$ and $k_{max}$ in \eqref{eq:purification_avg} can be determined from the results presented in \cite{Deutsch96}.  



\begin{table}[t]
\footnotesize
\begin{small}
    \centering
    \small
    \footnotesize
    % \setlength{\tabcolsep}{1pt}
    \begin{tabularx}{\columnwidth}{X c c c c }
      \toprule
      {Param} &   {$\cK$} & {$w_k$}&$\lambda^k_u$ &$F^k_u$ \\
    \midrule
      {Value} & {$3$}  &  {Unif$[0.1,1.0]$} &Unif$[0.1,1.0]$& {Unif$[0.75,0.94]$} 
    \\
      \bottomrule
    \end{tabularx}
    \vspace{-0.02in}
    \caption{\label{tab:parameters_value} Parameters used in our experiments.}
    \vspace{-0.1in}
    \end{small}
\end{table}


\myparab{Heuristic path-selection schemes:}
\myparab{Running process}

For each flow, we compute potentially 15 paths using the k-shortest path algorithm proposed in \cite{yen1971finding} where $k$ is $5$. 
The paths can overlap. We compute the $k$-shortest path when the weight of links is 1, $\frac{1}{c_l}$, and $\frac{1}{c_l^2}$.  We solve the optimization problem \ref{problem:flow_optimization} using the IBM CPLEX solver \cite{cplex}.



The random distillation strategy in greedy approach is selected randomly in range [0.94,0.974,99] and the average is plotted. 

\subsection{GA vs. baseline algorithms:} 

Figure \ref{fig:evolution_of_egr_in_genetic_algorithm} shows the evolution of the entanglement generation rate (EGR) with different flows in the network. The lower the number of flows, the faster the convergence of the genetic algorithm. It is because the number of genes in each individual for higher flows is higher and the genetic algorithm needs more generations to find the best solution. 


\begin{figure}[t]
\centering
\includegraphics[scale=0.2]{img/QVPN_GA_and_greedy_schemesv2.pdf}
\caption{GA vs. baseline algorithms}
\label{fig:evolution_of_egr_in_genetic_algorithm}
\end{figure}


\subsection{GA vs. Search Space}

\myparab{Candidate path size:}

Now, we show how the genetic algorithm will converge when the size of possible values for each flow is changing. We use the setup of 3 paths for each flow and 

\myparab{Distillation strategies:}

\myparab{Flow size:}

\begin{figure*}[t]
\centering
\begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{img/QVPN_GA_affect_of_search_space_distillation_strategies.pdf}  
     % \vspace{-0.06in}
    \caption{Different available distillation strategies}
    \label{fig:QVPN_GA_affect_of_search_space_population_sizes}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{img/QVPN_GA_affect_of_search_space_pathsv2.pdf} 
    % \vspace{-0.06in}
    \caption{Different number of candidate paths}
    \label{fig:QVPN_GA_affect_of_search_space_paths}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{img/QVPN_GA_affect_of_search_space_flowsv2.pdf}
    % \vspace{-0.06in}
    \caption{Different number of flows}
    \label{fig:QVPN_GA_affect_of_search_space_flows}
\end{subfigure}

\caption{Evolution of EGR over 1000 generations when we have different distillation strategies (\ref{fig:genetic_affect_of_different_distilation_strategies}), different Gate noise values (\ref{fig:genetic_affect_of_different_alpha_values}) and when we have different number of flows in the network (\ref{fig:genetic_affect_of_different_gate_noises})   \label{fig:evolution_of_egr_in_genetic_algorithm_with_different_dis_alpha_gate_noise}}
\end{figure*}





\subsection{Convergence of GA and gradient-based scheme}

\begin{figure}
\centering
\includegraphics[scale=0.2]{img/QVPN_GA_GR_as_time_in_minutes.pdf}
\caption{Convergence of genetic and gradient-based algorithms}
\label{fig:QVPN_GA_GR_as_time_in_minutes}
\end{figure}


\subsection{Minimum rate constraint}


\begin{figure}
\centering
\includegraphics[scale=0.2]{img/QVPN_GA_with_minimum_rate_constraintv2.pdf}
\caption{Convergence of genetic algorithm with minimum rate constraint}
\label{fig:Convergence_of_ga_with_minimum_rate_constraint}
\end{figure}


% \begin{figure}[t]
% \centering
% \includegraphics[scale=0.2]{img/initializing_ga_with_different_schemes_5_workloadsv2.pdf}
% \caption{Initializing the genetic algorithm with different heuristic approaches}
% \label{fig:initializing_ga_with_different_schemes}
% \end{figure}






% \begin{figure}
% \centering
% \includegraphics[scale=0.2]{img/initializing_ga_with_different_schemes_different_workloadsv2.pdf}
% \caption{The effect of how many training workloads we training the gradient-based approach}
% \label{fig:initializing_ga_with_different_num_wks}
% \end{figure}

% \begin{figure*}[t]
% \centering
% \begin{subfigure}{.32\textwidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{img/genetic_affect_of_different_population_sizes.pdf}  
%      % \vspace{-0.06in}
%     \caption{Different population sizes}
%     \label{fig:genetic_affect_of_different_population_sizes}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{img/genetic_affect_of_different_paths.pdf} 
%     % \vspace{-0.06in}
%     \caption{Different number of paths}
%     \label{fig:genetic_affect_of_different_paths}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{img/genetic_affect_of_different_flows.pdf}
%     % \vspace{-0.06in}
%     \caption{Different number of flows}
%     \label{fig:genetic_affect_of_different_flows}
% \end{subfigure}

% \caption{Evolution of EGR over 1000 generations when we have different population sizes (\ref{fig:genetic_affect_of_different_population_sizes}), different number of paths for each flow (\ref{fig:genetic_affect_of_different_paths}) and when we have different number of flows in the network (\ref{fig:genetic_affect_of_different_flows})   \label{fig:evolution_of_egr_in_genetic_algorithm}}
% \end{figure*}





==> extra/evaluation.tex <==
\section{Evaluation}
\label{experiment}
In this section, we conduct experiments to evaluate different schemes for path selection. scheme is providing the most rate of entanglement? (2) In what setup edge level or end level purification is doing better? (3) Which property of a network can affect most the end-to-end entanglement generation for users?



Setup:
Initialize from Hop based end level 
Initialize from Hob-based edge level

Initialize from hop-based edge and end level randomly

Initialize randomly from candidate with edge level

Only edge-level candidate paths 

Only end-level candidate paths 

Both edge-level and end-level candidate paths 

With three different gate values 





\myparab{Network topologies:} In our evaluation, we use the topologies of a real networks\footnote{Note that, the choice of such topologies are inspired by classical Internet which may or may not be deployed for quantum networks of the future.} including the Dutch SURFnet network, taken from the Internet topology zoo \cite{knight2011internet} and different 2-D topologies.




Table \ref{tab:parameters_value} shows the value of different parameters used in our experiments. Table \ref{table:topology_charecteristics} specifies the characteristics of the topologies. 

% \eat{We set the rate of entanglement generation on each edge in all networks to a value randomly chosen between 200 and 1400.  The fidelity of each edge in the network is randomly chosen from the range [0.96,0.99].
% We set the number of time intervals to 10 ($|T|=10$) and the duration of each time interval ($\Delta$) is 20 seconds.}

\myparab{Purification and Swapping:} We assume all noisy mixed entangled states in the network are Werner states \cite{werner1989quantum}. In our experiments, we use the recurrence-based purification scheme as explained in Section \ref{sec:Preliminaries}. In particular, we use the DEJMPS protocol \cite{Deutsch96} for purification. The values of $p_k$ and $k_{max}$ in \eqref{eq:purification_avg} can be determined from the results presented in \cite{Deutsch96}. When a node performs a (noise-free) entanglement swap operation between two EPR-pairs with fidelities $F_1$ and $F_2$, the fidelity of the resulting state is $\frac{1}{4}+\frac{3}{4}*(\frac{4F_1-1}{3})(\frac{4F_2-1}{3})$ \cite{briegel1998quantum}. We compute the basic fidelity of a path in the same way. 



\begin{table}[t]
\footnotesize
\begin{small}
    \centering
    \small
    \footnotesize
    % \setlength{\tabcolsep}{1pt}
    \begin{tabularx}{\columnwidth}{X c c c c }
      \toprule
      {Topologies} &   {$|V|$} & {$|E|$}&Avg. Degree &Diameter \\
    \midrule
      {SURFnet} & {50}  &  {68} &2.7& {11} 
         \\
    \midrule
      {$G(50,0.0.5)$} & {50}  &  {67} &2.8& {9.3} 
    \\
    \midrule
      {$PA(50,2)$} & {50}  &  {96} &3.8& {4.9} 
    \\
      \bottomrule
    \end{tabularx}
    \vspace{-0.05in}
    \caption{\label{table:topology_charecteristics} Properties of network topologies used in evaluation.}
    \vspace{-0.1in}
    \end{small}
\end{table}


\myparab{Workload}

We select the flows in the network randomly and set the fidelity threshold of each flow uniformly randomly selected in the range [0.7,0.92]. 

\subsection{Evolution of EGR in genetic algorithm}

\myparab{Running process}

For each flow, we compute potentially 15 paths using the k-shortest path algorithm proposed in \cite{yen1971finding} where $k$ is $5$. 

The paths can overlap. We compute the $k$-shortest path when the weight of links is 1, $\frac{1}{c_l}$, and $\frac{1}{c_l^2}$.  

Figure \ref{fig:evolution_of_egr_in_genetic_algorithm} shows the evolution of the entanglement generation rate (EGR) with different flows in the network. We conduct the experiments using the IBM CPLEX solver \cite{cplex}. The lower the number of flows, the faster the convergence of the genetic algorithm. It is because the number of genes in each individual for higher flows is higher and the genetic algorithm needs more generations to find the best solution. 




\begin{figure*}
\centering
\begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{img/genetic_affect_of_different_population_sizes.pdf}  
     % \vspace{-0.06in}
    \caption{Different population sizes}
    \label{fig:genetic_affect_of_different_population_sizes}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{img/genetic_affect_of_different_paths.pdf} 
    % \vspace{-0.06in}
    \caption{Different number of paths}
    \label{fig:genetic_affect_of_different_paths}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{img/genetic_affect_of_different_flows.pdf}
    % \vspace{-0.06in}
    \caption{Different number of flows}
    \label{fig:genetic_affect_of_different_flows}
\end{subfigure}

\caption{Evolution of EGR over 1000 generations when we have different population sizes (\ref{fig:genetic_affect_of_different_population_sizes}), different number of paths for each flow (\ref{fig:genetic_affect_of_different_paths}) and when we have different number of flows in the network (\ref{fig:genetic_affect_of_different_flows})   \label{fig:evolution_of_egr_in_genetic_algorithm}}
\end{figure*}



\subsection{Multiple candidate paths for each flow}

Now, we show how the genetic algorithm will converge when the size of possible values for each flow is changing. We use the setup of 3 paths for each flow and 



\begin{figure}
\centering
\includegraphics[scale=0.2]{img/convergence_of_genetic_1_3_path_multiple_candidates.pdf}
\caption{Convergence of genetic algorithm with different candidate paths}
\label{fig:convergence_of_genetic_1_path_multiple_candidates}
\end{figure}




% \subsection{Initialization of genetic algorithm}

% We show the different percentages of the initial population being set from the base scheme it good. Figure \ref{fig:affect_of_initialization_on_ga_convergence} shows that the higher the initialization, the faster the convergence because the genetic algorithm already is starting with a good population. 


% \begin{figure}
% \centering
% \includegraphics[scale=0.44]{img/affect_of_initialization_on_ga_convergence.pdf}
% \caption{The effect of initialization in genetic algorithm convergence}
% \label{fig:affect_of_initialization_on_ga_convergence}
% \end{figure}









% \begin{figure}

%   % \begin{subfigure}{.22\textwidth}
%   %   \includegraphics[width=4.0cm]{img/convergence_of_genetic_gradient_150_flows.pdf}
%   %   % \vspace{-0.2in}
%   % \caption{10 flows\label{fig:convergence_of_genetic_gradient_10_flows}}
%   % \end{subfigure}
%   \begin{subfigure}{.22\textwidth}
%     \includegraphics[width=4.0cm]{img/convergence_of_genetic_gradient_150_flows.pdf}
%     \caption{150 flows \label{fig:convergence_of_genetic_gradient_150_flows}}
%   \end{subfigure}
%   \caption{Convergence of genetic and gradient-based algorithms \label{fig:convergence_of_genetic_and_gradient_nased}}
% \end{figure}


\subsection{Initializing the genetic algorithm}

Figure \ref{fig:initializing_ga_with_different_schemes} shows that the gradient-based approach can be used as an initialization heuristic to generate the initial population of the genetic algorithm and it does better than other schemes. 

\begin{figure}
\centering
\includegraphics[scale=0.2]{img/initializing_ga_with_different_schemes_5_workloads.pdf}
\caption{Initializing the genetic algorithm with different heuristic approaches}
\label{fig:initializing_ga_with_different_schemes}
\end{figure}


\subsection{Convergence of genetic and RL scheme}

\begin{figure}
\centering
\includegraphics[scale=0.2]{img/convergence_of_genetic_gradient_150_flows.pdf}
\caption{Convergence of genetic and gradient-based algorithms}
\label{fig:convergence_of_genetic_and_gradient_nased}
\end{figure}


\begin{figure}
\centering
\includegraphics[scale=0.2]{img/initializing_ga_with_different_schemes_different_workloads.pdf}
\caption{The effect of how many training workloads we training the gradient-based approach}
\label{fig:initializing_ga_with_different_num_wks}
\end{figure}

\subsection{Initializing the genetic algorithm}

Figure \ref{fig:initializing_ga_with_different_schemes} shows that the gradient-based approach can be used as an initialization heuristic to generate the initial population of the genetic algorithm and it does better than other schemes. 

\eat{
\subsection{End-level or edge-level purification}

In this experiment, we evaluate the affect of doing edge level or end level on EGR.


\subsection{Sensitivity analysis}

In this experiment, we evaluate the sensitivity of different parameters of a network on final entanglement generation rate. 

\myparab{Process:} We express a link’s entanglement generation rate as $\frac{p_{elem}}{T}=\frac{2c\eta\alpha}{T}$.
The constant repetition times of $T$ is estimated from reference \cite{dahlberg2019link}. The non-fiber inefficiencies coefficient c is set to one.

\myparab{Expectation}

We plot average EGR for a different set of 6 user pairs in different networks using different path selection schemes as a function $\alpha$. Figure \ref{fig:EGR_as_alpha} shows that there is a value of $\alpha$ that we can have the highest EGR in the network. The function of EGR as a function of $\alpha$ would depend on the fidelity threshold of The relation between reduction in the rate of ELL pairs and less purification overhead comparing the high purification overhead.

}

\eat{\subsection{flexibility and Robustness}

QUESTION: Does an entanglement routing schedule (RS)
for all demands (source-destination pairs) exist in the network,
such that the number of entangled paths between any sourcedestination pair is not less than k?}

% \begin{figure}
% \centering
% \includegraphics[scale=0.44]{img/EGR_as_alpha.pdf}
% \caption{EGR as a function of $\alpha$.}
% \label{fig:EGR_as_alpha}
% \end{figure}




\subsection{Explaning state action space}



\subsubsection{State space}In our approach, at each given time $t$, the DRL agent observes the set of flows.

\subsubsection{Action space}For each state $s_t$, the agent feeds the value of the previous parameters to the neural network and outputs the action, i.e., the probability of selecting different paths. The top $|R|$ paths with the highest probabilities would be used for the next $w$ time intervals.





\subsubsection{Reward}For each set of suggested paths by the DRL agent, we solve the optimization problem (\ref{cons:optimal2}) to find the EGR. We use this EGR as our reward value.

%We compute the reward as $\frac{mlu^{optimal}}{mlu^{RL}}$ where $mlu^{optimal}$ is the average maximum link utilization for the optimal offline scheme (optimization problem \ref{cons:rate_constraint2}) over $w$ time intervals. Note that the optimal offline scheme at each time interval $t$ knows the future traffic matrices in the next $w$ time intervals. 



$\Delta\theta=  \alpha (\Delta\theta \log \pi (a_{t,R}|s_t;\theta)(r_t)+\beta\triangledown_{\theta} H(\pi(.|s_t;\theta)))$


==> extra/extra_formulations.tex <==

The problem formulation \ref{problem:flow_optimization} assumes the set of paths is given. We can rewrite the problem (\ref{problem:flow_optimization}) as follows:
\begin{align} 
\max_{x^k_p,y_p}  &\sum_{k\in \cK}\sum_{u\in U_k} \sum_{p\in \tilde{P}^{k}_u} w_k y_p x^k_p  \lambda^k_{u}
\nonumber
\\
\text{s.t.}& 
\nonumber\\
& \sum_{\substack{k \in \cK \\
{u \in U_k}\\
{p \in \tilde{P}^{k}_u}|l \in p}} x^{k}_p y_p \lambda^k_u h(F_p,F^k)  \leq c_l
\label{cons:edge_constraint2}, \quad l\in E\\
\quad & \sum_{p \in \tilde{P}^{k}_u} y_p \geq 1 \quad  \forall{k \in \cK \& u\in U_k} \\
\quad & \sum_{\substack{k \in \cK \\
{u \in U_k}\\
{p \in \tilde{P}^{k}_u}}} y_p \leq R \\
\quad & x^k_{p}\geq0,y_p\in\{0,1\}  \quad k \in \cK, u \in U_k, p \in \tilde{P}^{k}_u
\label{cons:variable_constraint2}
\end{align}

where we force all the flows to use at most $R$ paths and each flow should at least use one path. Here $\tilde{P}^{k}_u$ is the set of all possible paths in the network for user pair $u$ from the organization $k$. The binary variable $y_p \in \{0,1\}$ for each path $p$ indicates if that path has been used or not.



\begin{align} 
\max_{\Delta}  & \quad \Delta
\label{problem:flow_delta_optimization}
% \nonumber
\\
\text{s.t.}& 
\nonumber\\
& \sum_{\substack{k \in \cK \\
{u \in U_k}\\
{p \in P^k_{u}}|l \in p}} x^{k}_p g(F_p,F^k_u)  \leq c_l
\label{cons:edge_constraint_delta}, \quad l\in E\\
\quad & \sum_{p\in P^k_u} x^k_p \geq \Delta \lambda^k_u\\
\quad & \Delta \geq 0\\
\quad & x^k_{p}\geq0,  \quad k \in \cK, u \in U_k, p \in P^k_{u}
\label{cons:variable_constraint_delta}
\end{align}





where constraint \ref{cons:edge_constraint} is for edge capacity constraint. 


\begin{align} 
\max_{x^k_p}  &\sum_{k\in \cK}\sum_{u\in U_k} \sum_{p\in P^k_{u}} w_k x^k_p \lambda^k_{u} q^{|p|-1}
\label{problem:flow_optimization}
% \nonumber
\\
\text{s.t.}& 
\nonumber\\
& \sum_{\substack{k \in \cK \\
{u \in U_k}\\
{p \in P^k_{u}}|l \in p}} x^{k}_p \lambda^k_u g(F_p,F^k) + g(F_l,F^{th}_l)  \leq c_l
\label{cons:edge_constraint}, \quad l\in E\\
\quad & x^k_{p}\geq0,  \quad k \in \cK, u \in U_k, p \in P^k_{u}
\label{cons:variable_constraint}
\end{align}


\eat{When users are restricted to only one path each, we can obtain a significant reduction in variables. Let $p_u$ denote the path for user $u$. Interpret the weight $\lambda^k_u$ as follows. Let $x^k$ denote the aggregate EGR for organization $k$ across all of its users and let $x_u\lambda^k_u$ denote the EGR received by user $u\in U_k$. The weighted EGR maximization problem is
\begin{align} 
\max_{x^k}  &\sum_{k\in \cK}\sum_{u\in U_k}  w_k x^k \lambda^k_{u}
\nonumber
\\
\text{s.t.}& 
\nonumber\\
& \sum_{\substack{k \in K \\
{u \in U_k |l \in p_u}}} x^{k} \lambda^k_u h(F_{p_u},F^k)  \leq c_l, \quad l\in E \label{cons:edge_constraint2}\\ 
& x^k\geq 0,  \quad k \in \cK.
\label{cons:variable_constraint2}
\end{align}}


$K$ organizations use the same resources. Each organization has a weight indicated by $w_k$ and each user pair $(v,w)$ in organization $k$ has a weight indicated by $\lambda^k_{(v,w)}$. We assume that $U_{k_1}$ and $U_{k_2}$ can share users as well and that $U_{k_1} \cap U_{k_2}\neq \emptyset$. $x_k$ does not have a physical meaning by itself.


\subsection{flexibility and Robustness}

QUESTION: Does an entanglement routing schedule (RS)
for all demands (source-destination pairs) exist in the network,
such that the number of entangled paths between any source destination pair is not less than k?


\subsection{Ratio to network capacity}

As a function of number of paths between source destinations. The ration should increase as we add more paths to the network. 

\subsection{Sanity check}

We sanity check if the modified Wenhan's model for maximizing the EGR between a set of flows is truly compute the optimal rate. For that we assume a pair of users in a network. We assume the network can provide at most three paths. In our other setup, we assume that are connected to each other through one, two, and three completely disjoint paths. The result of two optimization should be equal. 

\section{Utility maximization}


The ideas from online learning  and online knapsack problem to admit or reject requests in the network.
We assume a discrete-time model where the time is divided
into  timeslots $t = 1,2,..$ and the $t$-th
request for entanglement generation arrives at the beginning of timeslot $t$. Each request $t$ has a source node $s_t$, destination node $d_t$, maximum EPR rate $demand_t$, and a set of candidate paths $P_t$. Each request may stay in the network for a few time slots and has a utility function that is a weighted sum of throughput and fidelity of the delivered EPR pairs for that request. 

Let $x^t_{p}$ be the raw entanglement rate delivered on path $p$ for request/flow $t$
 and $n^t_{p}$ rate on path $p$ for purifying pairs on path $p$ for request/flow $t$. Given $n^t_{p}$, function $f$ will return $1$ high quality EPR pair with fidelity $f$ on path $p$.
 
One possible utility function is then \\\\
$U_t = w_1 \frac{\log \sum_{p\in P_t} x^t_{p}}{d(t)} + w_2 \log \sum_{p\in P_t}f(n^t_{p})$ \\

where $w_1$ and $w_2$ are nonnegative scalars and indicate the
importance weight of the performance metrics. We use $\log$ to handle the fairness between requests. For throughput-sensitive requests, $w_1$ and $w_2$ are 1 and
0 respectively. For throughput-fidelity-sensitive requests, $w_1$ and $w_2$ are 0.5 and 0.5 respectively. For fidelity-sensitive requests, $w_1$ and $w_2$ are 0.0 and 1.0 respectively. 


Since throughput and Fidelity have very different scales, we normalize the throughput value of a request by the request’s maximum EPR rate $demand_t$. We define the throughput ratio for a request $t$ as the raw throughput value divided by the corresponding $demand_t$.

The goal is to maximize average utility of requests  as $maximize \quad  \lim_{T\to\infty}\frac{1}{T} \sum_{t=1}^T U_t$.




\subsection{Single-path case}

In this case, there is only one path between each user pair $u$.



\begin{table}
    \setlength{\tabcolsep}{3.5pt}
    \begin{tabularx}{\columnwidth}{c X }
      \toprule
      
      $G(V,E)$& A graph with $|V|$ nodes and $|E|$ edges
      \\
      \\
      {$c(u,v)$} & {Capacity of link $(u,v)$ in EPRs/sec}  \\ 
\\
% $K$ & Set of user pairs\\
        % \\
            $K$ & Set of organizations
    \\
    \\
     $U_k$ $\subset V\times V$ & set of user pairs in organization $k$
    \\
    \\
    $w_k$ & Weight of organization $k$
    \\
    \\
    $\lambda^k_{u}$ & Weight of user pair $u\in U_k$ in organization $k$
    \\
    \\
    
    
        % {$P^{k}_{u}$}  & {Set of paths connecting  user pair ${u}$ from organization $k$}  \\
        % \\
        % $F_p$ & Basic fidelity of path $p$\\
        % \\
          {$F^{k}$}  & Fidelity threshold of organization $k$  \\
        \\
        %   {$w^{k}$}  & Weight of user pair $k$  \\
        % \\
        $h(F^{th})$ & Avg. no. of base EPR pairs needed for purification to achieve fidelity threshold $F^{th}$\\
        \\
    % {$D^{k}$}  & {Rate of demand for request pair $k$ }   \\
    % \\

   
    % $\Delta_k$ & Relative weights, set of paths weights
    % \\
    % \\

%          {$F_{p}$}  & {Basic fidelity of path $p$ } 
%                     \\ 
% \\
\toprule
$x^{k}$ & Rate of entanglement generation for organization $k$
% \\ 
% \\
% $n_{p}^{k}$ & Number of purification rounds on path $p$ for user pair $k$
\\ 
\\
% $g(F_p,n^k_p)$ & the avg number of base EPR pairs used to perform $n^k_p$ number of consecutive successful purification rounds \\
% \\

    %   $f(.)$ & purification scheme
    %   \\
\hline
        
      \bottomrule
    \end{tabularx}
    \caption{\label{table:notaions} Notations used in the formulation.}
\end{table}

\begin{align} 
\max_{x^k}  & \sum_{k\in K}\sum_{u\in U_k} w_k x^k \lambda^k_{u}
\nonumber
\\
\text{subject to}\quad
\nonumber\\
\quad & \sum_{\substack{k \in K \\
{u \in U_k} }} x^{k} \lambda^k_u h(F^k)  \leq c(u,v)
\label{cons:edge_constraint} \quad {\forall{(u,v)}\in E}\\
\quad & x^k\geq0  \quad {k \in K \& u \in U_k }
\label{cons:variable_constraint}
\end{align}


\subsection{Routing and purification solution}

For reach arrived request $t$, we need to identify two things for each node in the network with respect to the link capacities and maximization of the total utility. First, how many EPR pairs to deliver (the throughput) and how much of the edge capacity on the outgoing links associated with the set of paths of that request should be allocated for the purification task. In this way, we obtain the routing and purification solution for the request.



\begin{align} 
\max_{x^t_{p},n^t_p}  &\lim_{T\to\infty}\frac{1}{T} \sum_{t=1}^T U_t
\nonumber
\\
\text{subject to}\quad
\nonumber\\
\quad & \sum_{\substack{t \in \text{running requests} \\
{p \in P^t}|(u,v) \in p}} x^{t}_{p}  n^t_{p}  \leq c(u,v)
\label{cons:edge_constraint} \quad {\forall{(u,v)}\in E}\\
\quad & \text{each request does not run more than $\tau$ (asked duration)} \\ 
\quad & \text{each request uses $\tau$ consecutive time slots} \\ 
\quad & x_{p}^{t}\geq0 \quad n^t_p\geq 1  \quad {k \in K}, {p\in P^{k}}
\label{cons:variable_constraint}
\end{align} 





\subsection{Maximizing EGR}

\begin{align} 
\max_{x^k_{p}}  & \quad\frac{1}{|K|}\sum_{k\in K}\sum_{p\in P^k}w^k  x^k_{p}
\nonumber
\\
\text{subject to}\quad
\nonumber\\
\quad & \sum_{\substack{k \in K \\
{p \in P^k}|(u,v) \in p}} x^{k}_{p}  h(F_p,F^k)  \leq c(u,v)
\label{cons:edge_constraint} \quad {\forall{(u,v)}\in E}\\
\quad & x_{p}^{k}\geq0  \quad {k \in K}, {p\in P^{k}}
\label{cons:variable_constraint}
\end{align} 

\section{Network Model}

In this section, we first explain the network model and then define the problem of resource allocation and load balancing on quantum storage servers in quantum networks. The notations used in this section are shown in Table \ref{table:notaions}.


Suppose that a central controller needs to continually establish end-to-end paths in the network to meet a dynamically changing demand in an online manner over a time horizon T . Let $K_t \in R$
 be the  set of requests  at timeslot $t$; let $P_t \in P$ be the set of paths that the controller establish in the network for time slot $t$. With establishing the set of  $P_t$, the controller observes two types of quality parameters: (i) The fidelity experienced by applications and (ii) switching costs that shows how many new paths it need to install in the network.
\myparab{Fidelity costs:} such as the monetary cost of reserving and using virtual machines, amortized
capital costs and energy expenditure to run local resources, as well as delay cost (revenue loss,
penalty for SLA violations). The parameter c balances the cost between power consumption and
average response time.

\myparab{Switching costs:} such as wear and tear and delay from startup and shutdown of servers, as well
as cost due to virtual machine migration and data transfer. Depending on the type of resource and
risk aversion of the service provider, the cost of changing resource allocations can be equivalent to
running them continually for a few minutes to several hours [10, 21, 48]. We model these costs
with a general norm of the difference in the consecutive provisioning decisions α ∥xt −xt−1 ∥ where
α represents the unit cost of change decisions.

\myparab{Network}

We consider the network as a graph $G = (V, E)$, where $V$ represents the set of nodes and $E$ abstracts the set of physical communication links. We define $c(u,v)$ as edge $(u,v)$ capacity, which denotes the maximum elementary EPR-pair generation rate with Fidelity $F$ in one time interval. We assume each pair of $(src,dst)$ nodes in the network have a set of predefined paths between each other indicated by $P^{(src,dst)}$.

\myparab{Workload}


We consider a discrete-time model whose timeslot matches the timescale at which resource management decisions must be taken. There are $K$ source-destination pairs that generate entanglement generation requests at each time interval. $D^{k}_{t}$ is the request rate from source-destination pair $k$ at time interval $t$. 



\begin{table}
    \servering
    \setlength{\tabcolsep}{3.5pt}
    \begin{tabularx}{\columnwidth}{c X }
      \toprule
      {$c(u,v)$} & {Capacity of link $(u,v)$}   \\ 
\\
% {$c_{e}$} & {Cost of link $e$}   \\ 
% \\
         {$P_{real}^{(src,dst)}$}  & {Set of all real paths between nodes $src$ and $dst$}  
        \\
        %   {$P^{s,h}$}  & {Set of all paths between storage pair $s,h$ where $\{s,h\} \in S $}  \\
        % \\
        $K_t$ & Set of requests at time interval $t$\\
                    \\
    {$D_{t}^{k}$}  & {Demand for request pair $k$  at time interval $t$}   \\

         {$F_{t}^{p}$}  & {Fidelity for path $p$ at time interval $t$} 
                    
      \bottomrule
    \end{tabularx}

    \caption{\label{table:notaions} Notations used in the paper.}
\end{table}



\myparab{Fidelity of each path and purification}

Due to the limitation of physical equipment, the fidelity degrades with the distance of the quantum channel and also degrades with the multiple entanglement swappings. Purification can be used to increase the Fidelity of established pairs between nodes. We use function $f_{scheme}(N,M)$ to show that in the purification scheme $scheme$, $N$ number of pairs are used in the purification process to generate $M$ high-quality bell pairs ($N>M$). The Fidelity value of the generated pairs is defined by this function. It is increasing in $N$ and decreasing in $M$. If we fix $M$, then by increasing $N$, we will get higher quality $M$ pairs.  On the other hand, the more bell pairs we generate from a fixed $N$ number of pairs, the lower the quality will be. Different versions of $f$ can either do the purification at the end node or each intermediate edge.   

\subsection{Maximizing fidelity}

\subsection{Maximizing aggregate end-to-end fidelity}

In this application, the arrived requests do not have a fidelity threshold and the goal is to maximize the average fidelity of served EPR pairs to users. QONs can use the stored EPR pairs at storage servers to purify the delivered EPR pairs to users. We use $n^k_{p,t}$ to indicate the number of EPR pairs that are used on path $p$ at time interval $t$ for user pair $k$ to generate one high quality EPR pair. If function $f$ represents the purification scheme, then the objective function is to maximize the average fidelity served to user pairs over T time intervals. We can write this as follows: \\

$F = \frac{1}{|T|}\sum_{t\in T}\frac{1}{|K_t|}\sum_{k\in K_t}\frac{1}{D_t^k}\sum_{p\in P^k_{N\cup S}}w^k_{p,t} f(p,n^k_{p,t})$.

In this problem formulation, our decision variables are $w^k_{p,t}$ and $n^k_{p,t}$. The problem formulation for this application for the infinite time intervals for EPR pairs life time extreme is as follows:

\begin{align} 
\max_{w^k_{p},n^k_{p}}  & \quad\frac{1}{|K|}\sum_{k\in K}\frac{1}{D^k}\sum_{p\in P^k}w^k_{p} f(p,n^k_{p})
\nonumber
\\
\text{subject to}\quad
\nonumber\\
\label{cons:demand_constraint}
\quad & \sum_{ p \in P^{k}}x_{p}^{k} =D^{k}   \quad  { \forall{k}\in K}\\
\nonumber \\
\quad & \sum_{\substack{k \in K \\
{p \in P^k}|(u,v) \in p}} x^{k}_{p}  n^k_p  \leq c(u,v)
\label{cons:edge_constraint} \quad {\forall{(u,v)}\in E}\\
\quad & x_{p}^{k}\geq0  \quad n^k_p\geq1 \quad {k \in K}, {p\in P^{k}}
\label{cons:variable_constraint}
\end{align} 




\begin{align} 
\max_{w^k_{p},n^k_{p,e}}  & \quad\frac{1}{|K|}\sum_{k\in K}\frac{1}{D^k}\sum_{p\in P^k}w^k_{p} f(p)
\nonumber
\\
\text{subject to}\quad
\nonumber\\
\label{cons:demand_constraint}
\quad & \sum_{ p \in P^{k}}x_{p}^{k} =D^{k}   \quad  { \forall{k}\in K}\\
\nonumber \\
\quad & \sum_{\substack{k \in K \\
{p \in P^k}|e \in p}} x^{k}_{p}  n^k_{p,e}  \leq c(e)
\label{cons:edge_constraint} \quad {\forall{e}\in E}\\
\quad & x_{p}^{k}\geq0  \quad n^k_{p,e}\geq1 \quad {k \in K}, {p\in P^{k}},\forall{e\in p}
\label{cons:variable_constraint}
\end{align} 


Note that the only difference between constraints in this problem formulation and constraints \eqref{cons:inventory_usage}
\eqref{cons:demand_constraint} \eqref{cons:edge_constraint}\eqref{cons:storage_capacity_constraint}\eqref{cons:variable_constraint}\eqref{cons:storage_variable_constraint} is that instead of having function $g(F_p,F_t^{k})$, we have variable $n^k_{p,t}$. 

\subsection{Problem formulation}

We use $F_t$ to show the average Fidelity at time interval $t$ and it is defined as $F_t=\frac{1}{|K_t|}\sum_{k\in K_t}F_{k,t}$. $F_{k,t}$ is equal to $\frac{1}{{D^k_t}}\sum_{p\in P^k}w^k_{p,t}* f(p,N^k_{p,t})$ where function $f$ would return the purified fidelity after using $N^k_{p,t}$ pairs on path $p$. For each request pair $k$ that uses the set of $P^k$ paths, we multiply the rate of entanglement generation rate at each path by the Fidelity of that path and divide it by the demand of that request pair ($D^k_t$). The problem formulation is as follows in equation \ref{equ:optimization}.





% F= $\frac{1}{T}\sum_{t\in T}\frac{1}{|K_t|}\sum_{k\in K_t}\frac{1}{{D^k_t}}\sum_{p\in P^k}w^k_{p,t} * \frac{F_p^2}{F_p^2+(1-F_p)^2}$
% \begin{equation}
% \begin{aligned}
% \max  F & \quad \\
% \textrm{s.t.} \quad &w_{p,t}^{k}\geq0 \quad  \forall{t}\& \forall{p\in P^{k \in \{K_t \cup J\}}}\\
% % \quad & N^{k}_{p,t}\geq1 \quad  \forall{t} \& \forall{k\in K_t}\& \forall{p\in P^{k \in \{K_t \cup J\}}}\\
% \quad & \sum_{\forall{p}|(u,v) \in p}\frac{2 w^{k}_{p,t}}{P_{succ}(p)} \leq c(u,v) \quad \forall{(u,v)\in E}\\
% % \quad & \sum_{p \in P^{k}|(u,v) \in p}w^{k}_{p,t} \leq c(u,v) \\
% % \quad & \quad \forall{(u,v) \in E}\& \forall{t} \& \forall{k \in \{K_t \cup J\}}\\
% %\quad & \sum_{p \in P^{s}}w^{p} \leq (C(s))  \quad \forall{s \in S}\\
% % \quad & \sum_{p \in P^{k}}w_{p,t}^{k}  N^{k}_{p,t} = D^{k}_{t} \quad \forall{t} \& \forall{k\in K_t}\\
% \quad & \sum_{p \in P^{k}}w_{p,t}^{k}  \geq D^{k}_{t} \quad \forall{t} \& \forall{k\in K_t}\\
% % \quad & \sum_{p \in P^{(s,h)}|h \in S \& (s,h) \in J}w_{p,t}^{k}  N^{k}_{p,t} \leq C_{s} \quad \forall{t} \& \forall{s \in S} \\
% \quad & \sum_{p \in P^{(s,h)}|h \in S \& (s,h) \in J}w_{p,t}^{(s,h)}  \leq C_{s} \quad \forall{t} \& \forall{s \in S} \\
% \quad & \sum_{p_1 \in P^k|(u,v)\in p_1}w^{k}_{p_1,t} \leq \sum_{p_2 \in P^{(u,v)}}w^{(u,v)}_{p_2,t-1} \quad \forall{(u,v) \in J \& \forall{k\in K}}
% \end{aligned}
% \label{equ:optimization}
% \end{equation}

% $max \sum_{t\in T}\sum_{k\in K}\sum_{p\in P}w^k_{p,t}f(p,n^k_{p,t})$

%F= $\sum_{t\in T}\sum_{k\in K_t} \sum_{p \in P^k}(\alpha y_{p,t} + \beta f(x_{p,t}))$


\begin{align} 
\min_{x^k_{p,t}}  & \sum_{t\in T}\sum_{k\in K_t} \sum_{p \in P^k}(\alpha y^k_{p,t} + \beta f(p,x^k_{p,t}))
\nonumber
\\
\text{subject to}\quad
& \quad \forall{t \in T:} \nonumber \\
\quad & y^k_{p,t} \geq |x_{p,t}^{k} -x_{p,t-1}^k| 
\label{cons:path_changing_cost} \quad \forall{k \in K, p \in P^k}  \\
\nonumber \\
\label{cons:demand_constraint}
\quad & \sum_{ p \in P^{k}}x_{p,t}^{k} =D^{k}_{t}   \quad  {k\in K_t}\\
\nonumber \\
\quad & \sum_{\substack{k \in K_t \\
{p \in P^k}|(u,v) \in p}} x^{k}_{p,t}  g(F_{(u,v)},F_p,F^k_t)  \leq c(u,v)
\label{cons:edge_constraint}
\nonumber \\
\quad & \quad \quad \quad  \quad \quad \quad \quad \quad \quad  \quad \quad \quad {(u,v)\in E}\\
\quad & x_{p,t}^{k}\geq0  \quad  {k \in K_t}, {p\in P^{k}}
\label{cons:variable_constraint}
\end{align} 





\subsection{Feasibility formulation}

% $t=1$\\
% $D^{(1,5)}_{t=0}\geq0$\\
% $P^{(1,5)}=\{[1,2,3,4,5],[1,2,4,5]\}$\\
% $P^{(2,4)} = \{[2,3,4]\}$\\
% $w^{(2,4)}_{p=\{2,3,4\},t=0} = 0$\\
% $w^{(1,5)}_{p=\{1,2,3,4,5\},t=0} = 0$\\
% \\
% $C(2,4) = w^{(2,4)}_{p=\{2,3,4\},t-1}$

We use below optimization problem (equation \ref{equ:feasibility_optimization}) to check  the feasibility of serving requests at each time interval. In this case, we do not have purification constraints.

\begin{equation}
\begin{aligned}
\max  \quad & 1\\
\textrm{s.t.} \quad &w_{p,t}^{k}\geq0 \quad  \forall{t}\& \forall{p\in P^{k \in \{K_t \cup J\}}}\\
% \quad & N^{k}_{p,t}\geq1 \quad  \forall{t} \& \forall{k\in K_t}\& \forall{p\in P^{k \in \{K_t \cup J\}}}\\
\quad & \sum_{p \in P^{k}|(u,v) \in p}w^{k}_{p,t} \leq c(u,v) \quad \forall{(u,v)\in E}\\
% \quad & \sum_{p \in P^{k}|(u,v) \in p}w^{k}_{p,t} \leq c(u,v) \\
% \quad & \quad \forall{(u,v) \in E}\& \forall{t} \& \forall{k \in \{K_t \cup J\}}\\
%\quad & \sum_{p \in P^{s}}w^{p} \leq (C(s))  \quad \forall{s \in S}\\
% \quad & \sum_{p \in P^{k}}w_{p,t}^{k}  N^{k}_{p,t} = D^{k}_{t} \quad \forall{t} \& \forall{k\in K_t}\\
\quad & \sum_{p \in P^{k}}w_{p,t}^{k}  = D^{k}_{t} \quad \forall{t} \& \forall{k\in K_t}\\
% \quad & \sum_{p \in P^{(s,h)}|h \in S \& (s,h) \in J}w_{p,t}^{k}  N^{k}_{p,t} \leq C_{s} \quad \forall{t} \& \forall{s \in S} 
\quad & \sum_{p \in P^{(s,h)}|h \in S \& (s,h) \in J}w_{p,t}^{(s,h)}  \leq C_{s} \quad \forall{t} \& \forall{s \in S} \\
% \quad & \sum_{p_1 \in P^k|(u,v)\in p_1}w^{k}_{p_1,t} \leq \sum_{p_2 \in P^{(u,v)}}w^{(u,v)}_{p_2,t-1} \quad \forall{(u,v) \in J \& \forall{k\in K}}
\end{aligned}
\label{equ:feasibility_optimization}
\end{equation}
 
 
 (P) is a convex optimization problem but the SP cannot
tackle it directly due to the following challenges:
• (Ch1): The user needs {ak} are unknown, time-varying and
possibly generated by a non-stationary random process.
• (Ch2): The spot {qk} and reservation prices {pt} are
unknown, time-varying and unpredictable as they depend on
the NO pricing strategy and possibly on other SPs’ demand.
• (Ch3): Finally, parameters qk and ak are revealed after the
slice reservation at the respective slot k has been decided.


. In
the case (S2), the necessary conditions for the environment can
be relaxed to V ({x∗
t }T
t=1 ) = o(T) and V ({gt}T
t=1 ) = o(T),
provided that a-priori knowledge of the environment is available. For example, when allocating resources to smart grids, the
temporal variations of the best dynamic solutions and instantaneous constraints can be estimated using day-ahead forecasting
of electricity loads and prices. Corollary 1 provides valuable insights for choosing optimal stepsizes in non-stationary settings.
Specifically, adjusting stepsizes to match the variability of the
environment is the key to achieving the optimal dynamic regret
and fit. Intuitively, when the variation is fast (a larger β), slowly
decaying stepsizes (thus larger stepsizes) can better track the
potential changes; and vice versa


 \subsection{Proposed algorithm}
 
 
 \subsubsection{cost}
 
 
 The cost is the final Fidelity. And the regret is the different between the optimal solution Fidelity over time and the Fidelity of our algorithm.
 
 
 One possible way of considering the switching cost is to purifying the stored qubits on some storage servers. In this way, turning on a server (purifying the qubits stored on it ) or turning it off (not using the qubits until they decohere) can be considdered as switching cost.
 
 
 Each storage server pairs have a cost. $Cost(j,M)$ indicates the cost of storing M qubits in the storage server pair $j$. This function can be extended to cover both the cost of storing and the cost of using the stored qubits by different pairs of nodes.  The demand is unknown. We use different algorithms to predict the demand in the future and compute an upper bound on the regret. The predictions on demands are from two angles: (i) first how much demand and then (ii) from which pair of nodes we will get the demands. We need to modify RHC and AFHC for this.
 
 
 \subsection{Prediction error and window}
 
 We need to consider the decoherence of qubits in the storage servers in the algorithm design.
 
 
 
 \myparab{High level of algorithm}
 The high-level goal of algorithms for OLIM is to store the asset when the
market price is cheap and use the stored asset when the price is expensive. However, the dynamics
of the prices and demand make this challenging. The main ideas that ARP uses to accomplish this
are: (i) adaptive reservation price based on inventory utilization, which tackles the challenges due
to price dynamics; and (ii) the construction of virtual inventories, which tackle the challenges due
to demand dynamics.




We use $P_y$ to show the set of paths that are used between storage servers. $P_x$ shows the set of paths between each source destination pair. At each time interval $t$, we need to decide on the rate of serving requests on paths in sets $P_x$ and $P_y$. We use $x_t$ and $y_t$ to show the rate of request serving on $P_x$ and $P_y$ respectively at time interval $t$. 

We want to maximize the Fidelity of requests in this time interval and in the next time interval. 




If the operator knew, at the beginning of each period $t$, the demands for the next time intervals, it could find the optimal t-period decision ($x^*_t$, $y^*_t$) by solving:

$N_t = \sum_{p\in P_t^{k}}^{} N_t^{p}(u,v)$  $\forall{k \in K}$

Each storage pair has a cost that indicates the number of purification pairs that is needed to be used to store some specific qubits. Different storage pair servers would have different costs.  Later the decoherence rate at each storage server pair can be involved in the cost of using that server. The cost of using storage server is also as a function of the affect that purifying and storing qubits on that storage pair has on the Fidelity of the requests served from the network. Because, generating and storing the qubits in the storage would affect the result for Fidelity in this round. 
\begin{algorithm}
\caption{Online resource allocation}\label{alg:algorithm1}
\KwData{Input:}
\KwResult{Output:}
 initialization\;
 \While{While condition}{
  instructions\;
  \eIf{condition}{
   instructions1\;
   instructions2\;
   }{
   instructions3\;
  }
 }
\end{algorithm}




\myparab{Evaluation}

In order to evaluate the performance of any proposed algorithm for this optimization problem, we use the competitive ratio. The competitive ratio of algorithm A is defined as the $regret(A)/regret(OPT)$, where $regret(A)$ is the objective function under our online proposed algorithm and $OPT$ is the optimal offline algorithm that has full knowledge of future.

==> extra/reading_list.tex <==
read these:

A Multiple-Entanglement Routing Framework for
Quantum Networks

Reconfigurable Quantum Internet Service Provider


Quantum Internet Protocol Stack: a Comprehensive Survey

Bayesian Optimization for Parameter Tuning in Evolutionary Algorithms

Genetic Algorithm Optimization
Applied to Electromagnetics:
A Review


Optimizing Resource Allocation for Virtualized
Network Functions in a Cloud Center Using
Genetic Algorithms

On Topology Design for the Quantum Internet

Entanglement purification and quantum error
correction

Maximizing Entanglement Routing Rate in
Quantum Networks: Approximation Algorithms

Alireza Shabani Cisco: Packet Switching in Quantum Networks: A Path to Quantum Internet


Building the quantum network*

Towards Quantum-resistant Virtual Private
Networks

Deploying an inter-European quantum network


Quantum Key Distribution: A Networking Perspective

Towards Large-Scale Quantum Networks


Concurrent Entanglement Routing for Quantum Networks:
Model and Designs

Experimental demonstration of entanglement delivery using a quantum network stack

Fragmentation-Aware Entanglement Routing for
Quantum Networks

A Heuristic Remote Entanglement Distribution
Algorithm on Memory-Limited Quantum Paths


Distributed Quantum Computing with QMPI

Connection-oriented and Connectionless Remote
Entanglement Distribution Strategies in Quantum
Networks


Online Entanglement Routing in Quantum Networks

Quantum Internet: from Medium Access Control to
Entanglement Access Control

Pre-Distribution of Entanglements in Quantum
Networks

A Multiple-Entanglement Routing Framework for
Quantum Networks

Multipath concurrent entanglement routing in
quantum networks based on virtual circuit

Multi-Entanglement Routing Design over
Quantum Networks

A Survey of Virtual Private LAN Services (VPLS): Past, Present and Future

Provisioning a Virtual Private Network:
A Network Design Problem for Multicommodity Flow

A Scalable VPN Gateway for
Multi-Tenant Cloud Services

Competitive caching with machine learned advice


Adaptive Joint Optimization of IT Resources and
Optical Spectrum Considering Operation Cost

Stochastic Network Utility Maximization
A tribute to Kelly’s paper published in this journal a decade ago

A Distributed CSMA Algorithm for Throughput and
Utility Maximization in Wireless Networks

Deterministic delivery of remote entanglement on a quantum network

Deterministic delivery of remote entanglement on a
quantum network

Dai, Wenhan, Tianyi Peng, and Moe Z. Win. "Quantum queuing delay." IEEE Journal on Selected Areas in Communications 38.3 (2020): 605-618.


Gyongyosi, Laszlo, and Sandor Imre. "Multilayer optimization for the quantum internet." Scientific reports 8.1 (2018): 1-15.

Multipath Routing for Multipartite State Distribution in Quantum Networks


Schoute, Eddie, et al. "Shortcuts to quantum network routing." arXiv preprint arXiv:1610.05238 (2016).

Online Optimization in Cloud Resource Provisioning:
Predictions, Regrets, and Algorithms
and

Read paper Online Linear Optimization with Inventory Management
Constraints

and 

Online Joint Optimization on Traffic Engineering
and Network Update in Software-defined WANs

and
Online Optimization in Cloud Resource Provisioning:
Predictions, Regrets, and Algorithms

Cost Minimizing Online Algorithms for
Energy Storage Management With
Worst-Case Guarantee

and

 Niv Buchbinder and Joseph Naor. 2009. Online primal-dual algorithms for covering and packing. Mathematics of
Operations Research 34, 2 (2009), 270–286.

and
 J. Lorenz, K. Panagiotou, and A Steger. 2009. Optimal algorithms for k-search with application in option pricing.
Algorithmica 55, 2 (2009), 311–328.


==> extra/unity_servers.tex <==

\eat{use myPython virtual interface that has Cplex installed on it on unity using:

source /work/spooryousefd_umass_edu/myPython/bin/activate


The first step is to login to a node:

$ srun --pty -p gypsum-titanx --gres=gpu:1 --mem=64G bash

Once you are assigned the node you need to know the IP address. Run:

$ ip -br addr
for juniper:
31
22
27
19

screen 410865.juniper_rl_moving_average2 on login2 or 1 for 1k population size

srun -c 6 -p cpu-long -t 14-0 --pty bash

source /work/spooryousefd_umass_edu/myPython/bin/activate


You can check how long your jobs are eligible to run with this:
squeue --me -O JobID,EndTime


One of the interfaces should have an address that looks like 10.100.x.x - copy that (leave off the /16 at the end).

After activating Anaconda, start the Jupyter server:

$ jupyter notebook --ip=<IP> --port=12345 --no-browser
    At the bottom of the output is a URL to use to access the notebook

To kill all screens :

screen -ls | grep Detached | cut -d. -f1 | awk '{print $1}' | xargs kill
From your laptop/desktop:

showing the screen name:
screen -X sessionname

$ ssh -L 12345:<IP address from earlier step>:12345 <username>@unity.rc.umass.edu

Then you should be able to use the URL generated by the Jupyter server (the one with 127.0.0.1) - paste it into a browser on your desktop/laptop.

sudo ssh -L 12345:10.100.10.1:12345 unity




command after you get a bunch of CPUs.


You cna use these commands to install a new one 

(base) spooryousefd_umass_edu@cpu009:~$ python -m venv /work/spooryousefd_umass_edu/myPython
(base) spooryousefd_umass_edu@cpu009:~$ source /work/spooryousefd_umass_edu/myPython/bin/activate
(myPython) (base) spooryousefd_umass_edu@cpu009:~$ mkdir /home/spooryousefd_umass_edu/build
(myPython) (base) spooryousefd_umass_edu@cpu009:~$ python /modules/apps/cplex/2210/python/setup.py build --build-base=/home/spooryousefd_umass_edu/build install --prefix=/work/spooryousefd_umass_edu/myPython/


if networkx is installed but you can not imprt it, use pipenv install networkx to install it in a virtual env. Sometimes networkx or other libraries do not detect the virtual environment.


}
